A Unifying Causal Framework for Analyzing Dataset Shift-stable Learning Algorithms

Recent interest in the external validity of prediction models (i.e., the problem of different train and test distributions, known as dataset shift) has produced many methods for finding predictive distributions that are invariant to dataset shifts and can be used for prediction in new, unseen environments. However, these methods consider different types of shifts and have been developed under disparate frameworks, making it difficult to theoretically analyze how solutions differ with respect to stability and accuracy. Taking a causal graphical view, we use a flexible graphical representation to express various types of dataset shifts. Given a known graph of the data generating process, we show that all invariant distributions correspond to a causal hierarchy of graphical operators which disable the edges in the graph that are responsible for the shifts. The hierarchy provides a common theoretical underpinning for understanding when and how stability to shifts can be achieved, and in what ways stable distributions can differ. We use it to establish conditions for minimax optimal performance across environments, and derive new algorithms that find optimal stable distributions. Using this new perspective, we empirically demonstrate that that there is a tradeoff between minimax and average performance.

==> sections/performance_theory.tex <==
\section{On the Performance of Stable Distributions}\label{sec:performance}
\input{figures/av.tex}

In this supplementary section we examine how the strength of a deleted edge affects the relative performance of stable model. This provides useful insights because, in general, it is possible to learn edge strengths from data.\footnote{Edge strengths correspond to natural direct effects which can be estimated if identifiable.} In particular, we will show there is a tradeoff between stability and performance under small shifts. To facilitate the analysis, we will consider linear SCMs and quantify how far a stable distribution is from achieving the highest achievable performance in a given environment (defined by edge strength). Note that in any given environment the optimal predictor (w.r.t. mean squared error (MSE)) is the conditional expectation $E[Y|\mathbf{O}]$ \citep{friedman2001elements}. Thus, we will define the \emph{regret} associated with a given environment to be the difference in performance between a stable predictor and the \emph{oracle} conditional expectation in that environment. 


We consider the form of a level 3 stable distribution since they generalize all stable distributions (Lemma \ref{lemma:level-three}) and have the greatest precision in removing singular edges (Corollary \ref{corollary:precision}): $P(Y|\mathbf{W}^*, \mathbf{Z})$, where $\mathbf{Z}\subseteq \mathbf{O}$ consists of observed variables and $\mathbf{W}^* \cap \mathbf{O} = \emptyset$ consists of counterfactual versions of observed variables \citep{subbaswamycounterfactual}. This means the only difference between a level 3 stable predictor ($E[Y|\mathbf{W}^*, \mathbf{Z}]$) and an oracle predictor is the feature set. Thus, regret reduces to a difference in performance attributable to the oracle's use of $\mathbf{X} = \mathbf{O}\setminus (\mathbf{Z})$, which includes factual versions of the $\mathbf{W}^*$. Note that in the linear case, counterfactuals take the form of \emph{auxiliary variables} (AVs) \citep{chen2016incorporating,chen2017identification}: modifications of observed variables in which the effects of some (or all) observed parents are removed. For example, in Fig \ref{fig:av}a we have the AV $W^* = W - \lambda_{xw} X$ which subtracts out the effect of $X$ on $W$. With respect to paths through $W^*$, the edge $X\rightarrow W$ is effectively removed. Thus, $P(Y|W^*,Z)$ is the optimal stable predictor since any additional conditioning (on $X$ or $W$) would activate unstable edge $\lambda_{yx}$.

To characterize regret,\footnote{We discuss the relation with some existing nonlinear results establishing when stable predictors are optimal in Appendix \ref{app:nonlinear}.} we first a stable predictor's MSE across environments. Then, we establish when the stable and oracle predictors have equal MSE.

\begin{restatable}
{theorem}{stablemse}\label{thm:stablemse}
For mean zero linear Gaussian SCMs, the MSE of a stable predictor is constant across environments.
\end{restatable}

\begin{restatable}
{theorem}{unstablezero}\label{thm:unstablezero}
Let $\mathcal{G}_0$ be the environment in which the coefficients associated with the unstable edges $E_u$ are all zero. In $\mathcal{G}_0$, the MSE of the oracle predictor $E_{\mathcal{G}_0}[Y|\mathbf{O}]$ is equal to the MSE of the optimal stable predictor $E_{\mathcal{G}_0}[Y|\mathbf{Z},\mathbf{W}^*]$.
\end{restatable}

The next result identifies environments for which the oracle MSE is lowest (and regret is highest).

\begin{restatable}
{lemma}{unstableinfty}\label{lemma:unstableinfty}
Suppose there is only one unstable edge $e$ with corresponding coefficient $\lambda$ and that this edge is active for the oracle predictor. As $|\lambda| \to \infty$ we have that the oracle MSE $\to 0$.
\end{restatable}

To visualize these results in the context of example Fig \ref{fig:av}a, in Fig \ref{fig:av}b we plot the MSE of the oracle predictor (blue) and stable predictor $E[Y|W^*,Z]$ (green) as we vary the strength of the unstable edge $\lambda_{yx}$. As we expect, the gap between the stable and oracle MSEs increases with the strength of the unstable edge. As a result, we lose the most information when the unstable association is strongest. 

The figure also demonstrates an important performance consequence of stable predictors. \textbf{Key Result:} There is a \emph{stability-performance tradeoff} between stability (and the ability to generalize well to new environments) and the performance in and near the training environment. In Fig \ref{fig:av}b the performance of the unstable predictor (red) $E[Y|W,X,Z]$ is better than the performance of the stable predictor for a range of environments corresponding to an interval (denoted by vertical dashed lines) surrounding the training value $\lambda_{yx}=5$ . Beyond this value, the unstable predictor's performance significantly and rapidly deteriorates, demonstrating poor generalization under large shifts. More generally, the results in Fig \ref{fig:av}b provide a useful visual characterization of the performance of stable and unstable predictors that makes it easy to reason about edge strengths, which we can learn from data, and can help us decide which invariances will be beneficial to enforce.
